Relaxing the Constraints of Clustered Planarity

In a drawing of a clustered graph vertices and edges are drawn as points and curves, respectively, while clusters are represented by simple closed regions. A drawing of a clustered graph is c-planar if it has no edge-edge, edge-region, or region-region crossings. Determining the complexity of testing whether a clustered graph admits a c-planar drawing is a long-standing open problem in the Graph Drawing research area. An obvious necessary condition for c-planarity is the planarity of the graph underlying the clustered graph. However, such a condition is not sufficient and the consequences on the problem due to the requirement of not having edge-region and region-region crossings are not yet fully understood. In order to shed light on the c-planarity problem, we consider a relaxed version of it, where some kinds of crossings (either edge-edge, edge-region, or region-region) are allowed even if the underlying graph is planar. We investigate the relationships among the minimum number of edge-edge, edge-region, and region-region crossings for drawings of the same clustered graph. Also, we consider drawings in which only crossings of one kind are admitted. In this setting, we prove that drawings with only edge-edge or with only edge-region crossings always exist, while drawings with only region-region crossings may not. Further, we provide upper and lower bounds for the number of such crossings. Finally, we give a polynomial-time algorithm to test whether a drawing with only region-region crossings exist for biconnected graphs, hence identifying a first non-trivial necessary condition for c-planarity that can be tested in polynomial time for a noticeable class of graphs.

==> makefile <==
finalname = journal

included_latex_sources = 
compiler = latex
psfiles = \


$(finalname): $(included_latex_sources) $(psfiles) $(finalname).tex
	$(compiler) $(finalname).tex

%.ps: %.fig
	fig2dev -Leps $< $@

%.ps: %.gif
	convert $< $@

%.ps: %.bmp
	convert $< $@

%.ps: %.jpg
	convert $< $@

startup:
	xemacs $(finalname).tex &
	xdvi $(finalname) &
	xfig -bg white -fg black &

clean:
	rm -f $(psfiles)
	rm -f $(finalname).ps
	rm -f tmp-data/*.avg
	rm -f tmp-data/*.txt
	rm -f src-data/*.tmp
	rm -f *~
	rm -f *.bak
	rm -f figures/*.bak
	rm -f *.toc
	rm -f *.aux
	rm -f *.blg
	rm -f *.dvi
	rm -f *.log
	rm -f *.bbl 
	rm -f *.idx 
	rm -f *.out 
	rm -f *.pdf
	rm -f *.thm
	rm -f *synctex

bib: 
	$(compiler) $(finalname).tex
	bibtex $(finalname)
	$(compiler) $(finalname).tex
	$(compiler) $(finalname).tex

ps: $(finalname)
	dvips -t a4 $(finalname).dvi -o # -pp 6 -t a4

#	dvips -t letter $(finalname).dvi -o

pdf: $(finalname)
	dvips -Ppdf $(finalname).dvi -o $(finalname).ps
	ps2pdf $(finalname).ps $(finalname).pdf

print: ps
	lpr -Ppolaris -h $(finalname).ps


